Trust Regions Sell, But Who's Buying? Overlap Geometry as an Alternative Trust Region for Policy Optimization

Standard trust-region methods constrain policy updates via Kullback-Leibler (KL) divergence. However, KL controls only an average divergence and does not directly prevent rare, large likelihood-ratio excursions that destabilize training--precisely the failure mode that motivates heuristics such as PPO's clipping. We propose overlap geometry as an alternative trust region, constraining distributional overlap via the Bhattacharyya coefficient (closely related to the Hellinger/Renyi-1/2 geometry). This objective penalizes separation in the ratio tails, yielding tighter control over likelihood-ratio excursions without relying on total variation bounds that can be loose in tail regimes. We derive Bhattacharyya-TRPO (BTRPO) and Bhattacharyya-PPO (BPPO), enforcing overlap constraints via square-root ratio updates: BPPO clips the square-root ratio q = sqrt(r), and BTRPO applies a quadratic Hellinger/Bhattacharyya penalty. Empirically, overlap-based updates improve robustness and aggregate performance as measured by RLiable under matched training budgets, suggesting overlap constraints as a practical, principled alternative to KL for stable policy optimization.

==> sections/e_experiments.tex <==
% \section{Evaluations and experiments}
% \subsection{MuJoCo environments}
% \label{subsec:mujoco}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/e_experiments/mujoco_returns.pdf}
%     \caption{MuJoCo.}
%     \label{fig:mujoco_all_envs_returns}
% \end{figure*}

% We benchmark BPPO and BTRPO on standard MuJoCo continuous-control tasks
% (\texttt{-v5} suite) \citep{todorov2012mujoco} and compare against two widely-used on-policy baselines:
% Proximal Policy Optimization (PPO) \citep{schulman2017ppo} and Trust Region Policy
% Optimization (TRPO) \citep{schulman2015trpo}.

% \textbf{Experimental Protocol.}
% To ensure statistical rigor and robustness to outlier seeds, we follow the
% evaluation recommendations of \citep{agarwal2021rliable}. For each algorithm--task
% pair, we train using \textbf{9 independent random seeds} and report the
% \emph{Interquartile Mean (IQM)} of final performance (higher is better). IQM is a
% robust aggregate statistic that downweights extreme outcomes, making it suitable
% for high-variance RL benchmarks.

% \textbf{Environments.}
% We evaluate on six MuJoCo tasks spanning different dynamics and difficulty:
% \texttt{Ant-v5}, \texttt{HalfCheetah-v5}, \texttt{Hopper-v5},
% \texttt{Humanoid-v5}, \texttt{InvertedPendulum-v5}, and \texttt{Walker2d-v5}.

% \begin{table}[t]
%     \centering
%     \caption{\textbf{MuJoCo IQM scores (9 seeds; higher is better).}
%     We report the Interquartile Mean (IQM) aggregated across 9 seeds for each
%     environment. Best per environment is bolded. The last row reports the mean
%     IQM across the six tasks (an unweighted average over environments).}
%     \label{tab:mujoco_iqm}
%     \begin{small}
%     \begin{sc}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lcccc}
%         \toprule
%         Environment & PPO & TRPO & BTRPO & \textbf{BPPO} \\
%         \midrule
%         Ant-v5               & \textbf{1470.8} & 816.7  & 1169.1 & 1293.9 \\
%         HalfCheetah-v5       & 3451.3 & 2819.2 & 3299.2 & \textbf{3856.3} \\
%         Hopper-v5            & 617.5  & 913.2  & 928.9  & \textbf{1321.6} \\
%         Humanoid-v5          & 147.5  & 204.9  & 110.2  & \textbf{1099.2} \\
%         InvertedPendulum-v5  & 977.4  & 992.8  & 979.6  & \textbf{997.0} \\
%         Walker2d-v5          & 1765.4 & 1076.7 & 1397.0 & \textbf{2697.3} \\
%         \midrule
%         \textbf{Mean IQM}    & 1405.0 & 1137.2 & 1314.0 & \textbf{1877.5} \\
%         \bottomrule
%     \end{tabular}}
%     \end{sc}
%     \end{small}
% \end{table}

% \textbf{Results and Analysis.}
% Table~\ref{tab:mujoco_iqm} shows that the proposed square-root surrogate is highly
% effective on MuJoCo:

% \begin{enumerate}
%     \item \textbf{BPPO improves robust performance on most tasks.}
%     BPPO attains the best IQM on 5/6 environments, with particularly large gains
%     on \texttt{HalfCheetah-v5}, \texttt{Walker2d-v5}, \texttt{Hopper-v5}, and
%     \texttt{Humanoid-v5}. This is consistent with our motivation: replacing the
%     raw importance ratio $r_\theta$ with $q_\theta=\sqrt{r_\theta}$ damps heavy-tail
%     updates while preserving a smooth learning signal, improving stability without
%     relying on hard clipping.

%     \item \textbf{BTRPO is competitive but more sensitive to penalty strength.}
%     BTRPO generally outperforms TRPO on several tasks (e.g., \texttt{Ant-v5},
%     \texttt{HalfCheetah-v5}, \texttt{Hopper-v5}, \texttt{Walker2d-v5}), but can be
%     less robust on \texttt{Humanoid-v5} under a fixed penalty coefficient $\beta$.
%     This suggests that while Hellinger regularization provides a principled
%     alternative to clipping, adaptive penalty tuning (or task-dependent $\beta$)
%     may further improve robustness on the hardest high-dimensional domains.
% \end{enumerate}

% \subsection{DM\_control environments}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/e_experiments/dm_returns.pdf}
%     \caption{DM.}
%     \label{fig:dm_all_envs_returns}
% \end{figure*}
% We evaluate the proposed geometric surrogates on the DeepMind Control Suite (\texttt{dm\_control}) \citep{tunyasuvunakool2020dm_control}, a benchmark characterized by high-dimensional continuous control tasks with complex contact dynamics. We compare BPPO and BTRPO against two standard on-policy baselines: Proximal Policy Optimization (PPO) \citep{schulman2017ppo} and Trust Region Policy Optimization (TRPO) \citep{schulman2015trpo}.

% \textbf{Experimental Protocol.} To ensure statistical rigor and mitigate the effects of outlier seeds, we adopt the evaluation recommendations of \citep{agarwal2021rliable}. We report results aggregated over \textbf{9 independent random seeds} per algorithm-task pair. Performance is quantified using the Interquartile Mean (IQM) and Optimality Gap. Metrics are computed over the final 10 evaluations of training to capture asymptotic convergence.

% \textbf{Environments.} We benchmark on five tasks of varying difficulty: \texttt{cartpole\_swingup}, \texttt{cheetah\_run}, \texttt{hopper\_hop}, \texttt{walker\_walk}, and the high-dimensional \texttt{humanoid\_walk}.

% % Requires: \usepackage{booktabs}

% \begin{table}[t]
%     \centering
%     \caption{\textbf{DM Control (9 seeds) IQM scores (higher is better).}
%     Interquartile Mean (IQM) aggregated across 9 seeds for each task.
%     Best per task is bolded. The last row reports the mean IQM across tasks.}
%     \label{tab:dm_control_scores}
%     \begin{small}
%     \begin{sc}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lcccc}
%         \toprule
%         Environment & PPO & BTRPO & TRPO & \textbf{BPPO} \\
%         \midrule
%          cartpole\_swingup & \textbf{806.21} & 799.39 & 804.93 & 778.72 \\
%          cheetah\_run      & 513.10 & 441.62 & 429.83 & \textbf{513.22} \\
%          hopper\_hop       & 0.91   & 0.69   & 0.57   & \textbf{13.23} \\
%          humanoid\_walk    & 1.98   & 1.88   & 1.47   & \textbf{2.10} \\
%          walker\_walk      & 656.94 & 626.75 & 550.04 & \textbf{673.23} \\
%         \midrule
%         \textbf{Mean IQM}  & 395.83 & 374.07 & 357.37 & \textbf{396.10} \\
%         \bottomrule
%     \end{tabular}}
%     \end{sc}
%     \end{small}
% \end{table}



% \textbf{Results and Analysis.}
% As detailed in Table~\ref{tab:dm_control_scores}, the proposed geometric surrogates
% remain competitive with standard on-policy baselines:

% \begin{enumerate}
%     \item \textbf{Asymptotic performance (BPPO).}
%     BPPO attains the highest IQM on \texttt{cheetah\_run}, \texttt{hopper\_hop},
%     \texttt{humanoid\_walk}, and \texttt{walker\_walk}, and achieves the best
%     overall \textbf{Mean IQM} across tasks. The largest improvement appears on
%     \texttt{hopper\_hop} (13.23 vs.\ 0.91 for PPO), indicating that the square-root
%     ratio geometry ($q_\theta=\sqrt{r_\theta}$) can preserve a useful learning signal
%     while damping extreme importance weights in high-variance regimes.

%     \item \textbf{BTRPO performance and stability trade-off.}
%     BTRPO is consistently competitive with PPO/TRPO and improves over TRPO on all
%     five tasks, but does not dominate PPO in this configuration (e.g., it trails PPO
%     on \texttt{cartpole\_swingup} and \texttt{cheetah\_run}). This suggests that while
%     the Hellinger penalty $\beta(1-q_\theta)^2$ provides a principled alternative to
%     clipping, its performance can be sensitive to the fixed penalty coefficient
%     on DM Control, motivating adaptive penalty tuning as future work.
% \end{enumerate}



% \subsection{Procgen environments}
% \label{subsec:procgen}

% We evaluate BPPO and BTRPO on the Procgen benchmark \citep{cobbe2020leveraging}, which
% measures robustness and generalization in procedurally-generated RL environments.
% Compared to continuous-control suites, Procgen tasks can induce higher stochasticity
% and variance due to level generation and sparse rewards, providing a complementary
% stress test for ratio-based policy-gradient updates.

% \textbf{Experimental Protocol.}
% We follow the standard Procgen evaluation setup with
% \texttt{distribution\_mode}=\texttt{easy},
% \texttt{start\_level}=10000,
% \texttt{num\_levels}=200, and
% \texttt{deterministic}=1.
% For each environment and algorithm, we train with \textbf{3 independent random seeds}.
% Each seed is evaluated for \textbf{25 episodes}, and we report the \emph{mean episode
% return across seeds} along with the \emph{standard deviation across seeds}.
% Given our extensive 9-seed evaluation on MuJoCo and DM Control, we treat Procgen as
% a complementary breadth benchmark under a smaller seed budget.
% (When duplicate runs exist for the same (env, algorithm, seed), we first average them
% within-seed.)

% \textbf{Environments.}
% We benchmark four Procgen tasks: \texttt{coinrun}, \texttt{heist}, \texttt{jumper},
% and \texttt{ninja}, all under the \texttt{easy} distribution.

% \begin{table}[t]
%     \centering
%     \caption{\textbf{Procgen (easy) aggregate performance (higher is better).}
%     Entries report mean episode return across 3 seeds $\pm$ std across seeds
%     (25 eval episodes/seed). Best per environment is bolded (ties bolded).}
%     \label{tab:procgen_easy_scores}
%     \begin{small}
%     \begin{sc}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lcccc}
%         \toprule
%         Environment & PPO & TRPO-KL & BTRPO-BC & \textbf{BPPO} \\
%         \midrule
%         CoinRun & 8.13 $\pm$ 1.29 & \textbf{9.20 $\pm$ 0.40} & 4.87 $\pm$ 4.69 & 8.53 $\pm$ 0.23 \\
%         Heist   & \textbf{1.87 $\pm$ 1.40} & 0.67 $\pm$ 0.46 & 0.67 $\pm$ 0.46 & \textbf{1.87 $\pm$ 1.40} \\
%         Jumper  & 4.67 $\pm$ 0.23 & 4.80 $\pm$ 1.06 & 5.73 $\pm$ 0.31 & \textbf{5.87 $\pm$ 1.80} \\
%         Ninja   & 6.27 $\pm$ 1.40 & \textbf{7.07 $\pm$ 1.01} & 4.27 $\pm$ 0.50 & 6.27 $\pm$ 2.20 \\
%         \bottomrule
%     \end{tabular}}
%     \end{sc}
%     \end{small}
% \end{table}

% \textbf{Results and Analysis.}
% Table~\ref{tab:procgen_easy_scores} reports aggregate returns on Procgen. Unlike the
% consistent gains we observe in continuous control, results on Procgen are more mixed,
% which we attribute to procedural stochasticity and task-specific reward structure:

% \begin{enumerate}
%     \item \textbf{BPPO remains competitive under procedural stochasticity.}
%     BPPO improves over PPO on \texttt{coinrun} and achieves the best performance on
%     \texttt{jumper}, while matching PPO on \texttt{heist}. This supports the central
%     intuition of our surrogate: using the square-root ratio $q_\theta=\sqrt{r_\theta}$
%     moderates large-ratio updates while preserving a smooth learning signal, which can
%     be beneficial in high-variance settings.

%     \item \textbf{BTRPO-BC can be sensitive to fixed penalty strength on Procgen.}
%     In our current configuration, BTRPO-BC exhibits substantially higher variance and
%     lower mean performance on \texttt{coinrun} and \texttt{ninja}. This suggests that a
%     non-adaptive penalty coefficient $\beta$ may require more careful tuning in Procgen,
%     where reward sparsity and heavier-tailed returns can amplify the trade-off between
%     overlap regularization and exploration.
% \end{enumerate}

\section{Evaluations and experiments}

\paragraph{Evaluation philosophy.}
Across continuous-control benchmarks, we emphasize robust reporting and matched budgets.
Unless noted otherwise, results are aggregated over multiple random seeds and summarized with
RLiable-style statistics (IQM and Optimality Gap) to reduce sensitivity to outlier runs
\citep{agarwal2021rliable}. We report learning curves (mean across seeds with shaded variability)
to highlight both asymptotic performance and training stability.

\subsection{MuJoCo environments}
\label{subsec:mujoco}

We benchmark BPPO and BTRPO on standard MuJoCo continuous-control tasks (\texttt{-v5} suite)
\citep{todorov2012mujoco} and compare against two widely-used on-policy baselines:
PPO \citep{schulman2017ppo} and TRPO \citep{schulman2015trpo}.

\textbf{Experimental Protocol.}
Following \citep{agarwal2021rliable}, for each algorithm--task pair we train using
\textbf{9 independent random seeds} and report the \textbf{Interquartile Mean (IQM)} of final
performance (higher is better). Learning curves in Figure~\ref{fig:mujoco_all_envs_returns} show the
average return trajectory over training, with shaded regions indicating across-seed variability.

\textbf{Environments.}
We evaluate on six MuJoCo tasks spanning different dynamics and difficulty:
\texttt{Ant-v5}, \texttt{HalfCheetah-v5}, \texttt{Hopper-v5}, \texttt{Humanoid-v5},
\texttt{InvertedPendulum-v5}, and \texttt{Walker2d-v5}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/e_experiments/mujoco_returns.pdf}
    \caption{\textbf{MuJoCo learning curves (9 seeds).}
Mean episodic return over training on six MuJoCo tasks; shaded regions indicate $\pm 1$ standard deviation across seeds.
BPPO generally achieves higher returns and more sustained late-stage improvement on harder locomotion tasks.}
\label{fig:mujoco_all_envs_returns}
\end{figure*}

\begin{table}[t]
    \centering
    \caption{\textbf{MuJoCo IQM scores (9 seeds; higher is better).}
    We report the Interquartile Mean (IQM) aggregated across 9 seeds for each
    environment. Best per environment is bolded. The last row reports the mean
    IQM across the six tasks (an unweighted average over environments).}
    \label{tab:mujoco_iqm}
    \begin{small}
    \begin{sc}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        Environment & PPO & TRPO & BTRPO & \textbf{BPPO} \\
        \midrule
        Ant-v5               & \textbf{1470.8} & 816.7  & 1169.1 & 1293.9 \\
        HalfCheetah-v5       & 3451.3 & 2819.2 & 3299.2 & \textbf{3856.3} \\
        Hopper-v5            & 617.5  & 913.2  & 928.9  & \textbf{1321.6} \\
        Humanoid-v5          & 147.5  & 204.9  & 110.2  & \textbf{1099.2} \\
        InvertedPendulum-v5  & 977.4  & 992.8  & 979.6  & \textbf{997.0} \\
        Walker2d-v5          & 1765.4 & 1076.7 & 1397.0 & \textbf{2697.3} \\
        \midrule
        \textbf{Mean IQM}    & 1405.0 & 1137.2 & 1314.0 & \textbf{1877.5} \\
        \bottomrule
    \end{tabular}}
    \end{sc}
    \end{small}
\end{table}

\textbf{Results and Analysis.}
Figure~\ref{fig:mujoco_all_envs_returns} and Table~\ref{tab:mujoco_iqm} show that the proposed square-root
geometry improves both \emph{learning dynamics} and \emph{robust aggregate performance} on MuJoCo.

\begin{enumerate}
    \item \textbf{BPPO yields stronger learning dynamics and the best overall aggregate.}
    BPPO achieves the best IQM on 5/6 environments and the highest \textbf{Mean IQM} across tasks
    (Table~\ref{tab:mujoco_iqm}). Importantly, the learning curves in Figure~\ref{fig:mujoco_all_envs_returns}
    suggest that these gains are not limited to final scores: BPPO typically exhibits
    \emph{faster early learning} and \emph{more sustained late-stage improvement} on the harder
    locomotion tasks. The separation is most pronounced on \texttt{Walker2d-v5} and
    \texttt{HalfCheetah-v5}, where BPPO maintains a clear advantage as training progresses, and on
    \texttt{Humanoid-v5}, where BPPO continues improving while PPO/TRPO plateau substantially.
    These dynamics align with the central contribution of our method: using the square-root ratio
    $q_\theta=\sqrt{r_\theta}$ damps extreme importance weights while preserving a smooth learning
    signal, enabling continued improvement in regimes where large-ratio excursions can otherwise
    destabilize or stall training.

    \item \textbf{Mechanistic evidence for tail control on \texttt{Humanoid-v5}.}
    Figure~\ref{fig:intro:humanoid:returns} provides a mechanistic view of the observed performance gap.
    As training progresses, PPO’s learning curve flattens while BPPO continues to improve, and this
    divergence coincides with a contraction of PPO’s likelihood-ratio statistics (both the mean and
    an upper-tail summary), whereas BPPO maintains near-unity mean ratios while still retaining a
    non-trivial upper tail. This supports the interpretation that overlap-based updates can
    \emph{preserve effective update magnitude} in high-dimensional control while still \emph{damping}
    extreme ratio excursions---a key motivation of the proposed geometry.

    \item \textbf{BTRPO is competitive and exhibits a conservative stability profile.}
    BTRPO improves over TRPO on several tasks (e.g., \texttt{Ant-v5}, \texttt{HalfCheetah-v5},
    \texttt{Hopper-v5}, \texttt{Walker2d-v5}) but is more sensitive on \texttt{Humanoid-v5} under a
    fixed penalty coefficient $\beta$ (Table~\ref{tab:mujoco_iqm}). The learning curves in
    Figure~\ref{fig:mujoco_all_envs_returns} are consistent with a more \emph{conservative} update profile:
    BTRPO often progresses steadily without the sharp jumps characteristic of clipping-based updates.
    These results indicate that the Hellinger penalty $\beta(1-q_\theta)^2$ offers a principled
    trust-region alternative, and suggest that adaptive penalty tuning (or dual adjustment of $\beta$)
    may further improve robustness on the hardest domains.
\end{enumerate}

\subsection{DM Control environments}
\label{subsec:dmcontrol}

We evaluate the proposed geometric surrogates on the DeepMind Control Suite
(\texttt{dm\_control}) \citep{Tassa2020dmcontrolSA}, a benchmark characterized by
continuous control with complex contact dynamics. We compare BPPO and BTRPO against PPO and TRPO
\citep{schulman2017ppo,schulman2015trpo}.

\textbf{Experimental Protocol.}
We follow \citep{agarwal2021rliable} and train \textbf{9 seeds} per algorithm--task pair.
We report IQM (Table~\ref{tab:dm_control_scores}) and provide learning curves
(Figure~\ref{fig:dm_all_envs_returns}) to expose both asymptotic performance and stability.

\textbf{Environments.}
We benchmark five tasks: \texttt{cartpole\_swingup}, \texttt{cheetah\_run},
\texttt{hopper\_hop}, \texttt{walker\_walk}, and \texttt{humanoid\_walk}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/e_experiments/dm_returns.pdf}
    \caption{\textbf{DM Control learning curves (9 seeds).}
Average episodic return vs.\ environment steps on five tasks; shaded regions indicate $\pm 1$ standard deviation across seeds.
BPPO shows stronger learning progress on \texttt{cheetah\_run}, \texttt{hopper\_hop}, and \texttt{walker\_walk}, while PPO remains competitive on \texttt{cartpole\_swingup}.}
    
    \label{fig:dm_all_envs_returns}
\end{figure*}

\begin{table}[t]
    \centering
    \caption{\textbf{DM Control (9 seeds) IQM scores (higher is better).}
    Interquartile Mean (IQM) aggregated across 9 seeds for each task.
    Best per task is bolded. The last row reports the mean IQM across tasks.}
    \label{tab:dm_control_scores}
    \begin{small}
    \begin{sc}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        Environment & PPO & BTRPO & TRPO & \textbf{BPPO} \\
        \midrule
         cartpole\_swingup & \textbf{806.21} & 799.39 & 804.93 & 778.72 \\
         cheetah\_run      & 513.10 & 441.62 & 429.83 & \textbf{513.22} \\
         hopper\_hop       & 0.91   & 0.69   & 0.57   & \textbf{13.23} \\
         humanoid\_walk    & 1.98   & 1.88   & 1.47   & \textbf{2.10} \\
         walker\_walk      & 656.94 & 626.75 & 550.04 & \textbf{673.23} \\
        \midrule
        \textbf{Mean IQM}  & 395.83 & 374.07 & 357.37 & \textbf{396.10} \\
        \bottomrule
    \end{tabular}}
    \end{sc}
    \end{small}
\end{table}

\textbf{Results and Analysis.}
Figure~\ref{fig:dm_all_envs_returns} and Table~\ref{tab:dm_control_scores} show that the proposed
square-root geometry yields consistent improvements in both \emph{learning dynamics} and
\emph{robust aggregate performance} on DM Control.

\begin{enumerate}
    \item \textbf{BPPO improves learning dynamics and achieves the best overall aggregate.}
    BPPO attains the highest IQM on \texttt{cheetah\_run}, \texttt{hopper\_hop},
    \texttt{humanoid\_walk}, and \texttt{walker\_walk}, and it achieves the best overall
    \textbf{Mean IQM} across tasks (Table~\ref{tab:dm_control_scores}). Beyond final scores,
    the learning curves in Figure~\ref{fig:dm_all_envs_returns} indicate that BPPO typically exhibits
    \emph{faster early improvement} and \emph{more stable late-stage training} than PPO/TRPO,
    with reduced oscillation in several tasks. The largest gain is on \texttt{hopper\_hop},
    where BPPO’s curve separates decisively from the baselines and maintains the lead, consistent
    with the method’s motivation: operating on the square-root ratio $q_\theta=\sqrt{r_\theta}$
    damps extreme importance weights while preserving a smooth update signal.

    \item \textbf{BTRPO provides a principled trust-region alternative, with a conservative update profile.}
    BTRPO exceeds TRPO on all five tasks in Table~\ref{tab:dm_control_scores}, and the curves in
    Figure~\ref{fig:dm_all_envs_returns} suggest a more \emph{conservative} update profile: BTRPO often tracks
    PPO early in training but improves more gradually and exhibits fewer sharp spikes, consistent
    with the smooth overlap penalty $\beta(1-q_\theta)^2$. While BTRPO does not dominate PPO in this
    configuration (e.g., \texttt{cartpole\_swingup}), its stability-oriented behavior supports the
    role of Hellinger regularization as a practical alternative to heuristic clipping, and motivates
    adaptive penalty tuning as future work.
\end{enumerate}


\subsection{Procgen environments}
\label{subsec:procgen}

We evaluate BPPO and BTRPO on the Procgen benchmark \citep{Cobbe2019LeveragingPG}, which measures
robustness and generalization in procedurally-generated RL environments. Compared to continuous
control, Procgen tasks can exhibit higher stochasticity and sparser rewards, providing a
complementary stress test for ratio-based updates.

\textbf{Experimental Protocol.}
We use \texttt{distribution\_mode}=\texttt{easy}, \texttt{start\_level}=10000,
\texttt{num\_levels}=200, and \texttt{deterministic}=1. For each environment and algorithm, we
train \textbf{3 seeds}; each seed is evaluated for \textbf{25 episodes}. We report mean episode
return across seeds $\pm$ std across seeds. Given our extensive 9-seed evaluation on MuJoCo and
DM Control, we treat Procgen as a complementary breadth benchmark under a smaller seed budget.

\textbf{Environments.}
We benchmark four Procgen tasks: \texttt{coinrun}, \texttt{heist}, \texttt{jumper}, and
\texttt{ninja}.

\begin{table}[t]
    \centering
    \caption{\textbf{Procgen (easy) aggregate performance (higher is better).}
    Entries report mean episode return across 3 seeds $\pm$ std across seeds
    (25 eval episodes/seed). Best per environment is bolded (ties bolded).}
    \label{tab:procgen_easy_scores}
    \begin{small}
    \begin{sc}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        Environment & PPO & TRPO-KL & BTRPO-BC & \textbf{BPPO} \\
        \midrule
        CoinRun & 8.13 $\pm$ 1.29 & \textbf{9.20 $\pm$ 0.40} & 4.87 $\pm$ 4.69 & 8.53 $\pm$ 0.23 \\
        Heist   & \textbf{1.87 $\pm$ 1.40} & 0.67 $\pm$ 0.46 & 0.67 $\pm$ 0.46 & \textbf{1.87 $\pm$ 1.40} \\
        Jumper  & 4.67 $\pm$ 0.23 & 4.80 $\pm$ 1.06 & 5.73 $\pm$ 0.31 & \textbf{5.87 $\pm$ 1.80} \\
        Ninja   & 6.27 $\pm$ 1.40 & \textbf{7.07 $\pm$ 1.01} & 4.27 $\pm$ 0.50 & 6.27 $\pm$ 2.20 \\
        \bottomrule
    \end{tabular}}
    \end{sc}
    \end{small}
\end{table}

\textbf{Results and Analysis.}
Table~\ref{tab:procgen_easy_scores} reports aggregate returns on Procgen. Unlike the consistent
gains in continuous control, results are more mixed, which we attribute to procedural stochasticity
and task-specific reward structure.

\begin{enumerate}
    \item \textbf{BPPO remains competitive under procedural stochasticity.}
    BPPO improves over PPO on \texttt{coinrun} and achieves the best performance on \texttt{jumper},
    while matching PPO on \texttt{heist} (Table~\ref{tab:procgen_easy_scores}). This supports the
    central intuition of the square-root surrogate: using $q_\theta=\sqrt{r_\theta}$ moderates
    large-ratio updates while preserving a smooth learning signal in high-variance settings.

    \item \textbf{BTRPO-BC shows higher sensitivity to fixed penalty strength on Procgen.}
    In our current configuration, BTRPO-BC exhibits higher variance and lower mean performance on
    \texttt{coinrun} and \texttt{ninja} (Table~\ref{tab:procgen_easy_scores}), suggesting that a
    non-adaptive penalty coefficient $\beta$ may require more careful tuning in Procgen where reward
    sparsity can amplify the exploration--stability trade-off.
\end{enumerate}

